Hardness of Graph-Structured Algebraic and Symbolic Problems

In this paper, we study the hardness of solving graph-structured linear systems with coefficients over a finite field $\mathbb{Z}_p$ and over a polynomial ring $\mathbb{F}[x_1,\ldots,x_t]$. We reduce solving general linear systems in $\mathbb{Z}_p$ to solving unit-weight low-degree graph Laplacians over $\mathbb{Z}_p$ with a polylogarithmic overhead on the number of non-zeros. Given the hardness of solving general linear systems in $\mathbb{Z}_p$ [Casacuberta-Kyng 2022], this result shows that it is unlikely that we can generalize Laplacian solvers over $\mathbb{R}$, or finite-element based methods over $\mathbb{R}$ in general, to a finite-field setting. We also reduce solving general linear systems over $\mathbb{Z}_p$ to solving linear systems whose coefficient matrices are walk matrices (matrices with all ones on the diagonal) and normalized Laplacians (Laplacians that are also walk matrices) over $\mathbb{Z}_p$. We often need to apply linear system solvers to random linear systems, in which case the worst case analysis above might be less relevant. For example, we often need to substitute variables in a symbolic matrix with random values. Here, a symbolic matrix is simply a matrix whose entries are in a polynomial ring $\mathbb{F}[x_1, \ldots, x_t]$. We formally define the reducibility between symbolic matrix classes, which are classified in terms of the degrees of the entries and the number of occurrences of the variables. We show that the determinant identity testing problem for symbolic matrices with polynomial degree $1$ and variable multiplicity at most $3$ is at least as hard as the same problem for general matrices over $\mathbb{R}$.

==> STOC22_review.tex <==
--------------

Review #98A
===========================================================================

Paper summary
-------------
Linear system solving over the reals is well-studied: In general it can be solved in matrix multiplication time, and for important special cases like Laplacian systems the running time can be improved to near-linear. Linear system solving is much less studied over finite fields. In particular, there are no big special cases that are known to be solvable in near-linear time. The paper tries to explain this situation: The main result is a reduction from general linear systems to Laplacian systems, and even unit weight Laplacian systems. This shows that over finite fields solving (unit weight) Laplacian systems is equally hard as general linear systems, up to logfactors. Let me discuss the two special cases studied in this paper:

* Laplacian systems: Over finite fields, Laplacian systems simply are matrices that have the all-ones vector in their kernel. This is a much less restrictive condition compared to a real matrix being Laplacian. It is thus not very surprising that over finite fields Laplacian systems are as hard as general linear systems. Indeed, the presented reduction from general to Laplacian systems is quite simple; see the last equation on page 12 for the complete reduction, and the next page for the correctness proof.

* Unit weight Laplacian systems: The paper defines "unit weight" in a slightly weird way. A natural definition, in my eyes, would be to require that each off-diagonal entry is 0 or -1 mod p. Their methods should apply to this definition as well. The reduction to this special case is much more involved than for Laplacians. The authors are building small "circuits" that can generate any resistance mod p, by combining serial and parallel repetition, and using some tricks involving all small primes.

Generally, the paper seems to be written in a hurry, and needs more polishing. While the question is interesting and some parts of the reduction are quite non-trivial, the definitions of (unit weight) Laplacians are much less natural over finite fields, and thus the main results are not very surprising.


* What is best about the paper: The paper poses the interesting question of whether the seminal Laplacian system solvers for real matrices have an analogue over finite fields, and answers it negatively.

* What are the paper's weaknesses: The definitions of "Laplacian" and "unit weight" are much less natural over finite fields, so it is kind of expected that these cases are hard over finite fields.

* The paper's target audience: People in continuous optimization that are wondering why their techniques don't apply to finite fields.

* Recommendation summary: Weak reject.

Comments for author
-------------------
- Why not simply define "unit weight" by requiring that every off-diagonal entry is 0 or -1 mod p? This seems to be a much more intuitive intuition, and your methods should be able to reduce to this case.

- The paper needs more polishing. E.g. in Section 2.4 you refer to Definition 10 for the definition of size(A), although it was just defined in Section 2.2.

- In the intro, clarify what you mean by "solving" a linear system. You mean approximation algorithms with a polylog(1/eps) dependence, is that right?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #98B
===========================================================================

Paper summary
-------------
Solving systems of linear equations is one of the most basic algorithmic tasks. The best algorithms for general linear systems run in time O(n^omega) where omega is the exponent of matrix multiplication.Faster algorithms are known in structured special cases, such as Laplacian graph systems over the reals.

In this paper the authors consider the problem over prime fields GF(p). Their main results are reductions between general linear system and Laplacian systems that roughly preserve the sparsity of the matrix of the linear system. Thus, any improved algorithms for sparse Laplacian systems will imply an improvement for the general problem.

Over GF(p) any symmetric matrix that has the all-1 vector in its kernel can be thought of as a Laplacian of a graph. Thus in some sense this class is much more powerful than over the reals (where in each case we compare the expressibility of Laplacian systems with general linear systems). So in this sense the results are somewhat unsurprising and indeed the reduction from the general case to the Laplacian case is fairly simple.

The authors then show that (up to a small blow-up) one can further reduce Laplacian systems to what they call unit-weight Laplacian systems.
In the unit-weight setting, one thinks of the matrix as the Laplacian of a (non-simple) graph whose edges all have unit weights, and tracks not only the number of non-zero entries in the matrix but the number of such edges in the graph (or in other words, the absolute values of the entries of the matrix when thought of as integers). The authors show that every linear system can be reduced to a system where the size in this model is at most roughly the number of non-zeros in the original system (up to a log^2(p)/log log p blow-up).

The proof for the general Laplacian case is particularly simple and direct. The proof for the unit-weight case involves an iterative application of certain "gadget" constructions, some of them are folklore over R but applied and reproved here for the GF(p) setting.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #98C
===========================================================================

Paper summary
-------------
## Paper summary
This paper considers solving systems of linear equations over finite fields Z_p.
The goal of the paper is to investigate whether linear equations in matrices with a special structure known as Laplacian or Unit-weight Laplacian are likely to have faster solvers than solvers for general matrices.
The authors show that this cannot be the case, as linear equations in Laplacians and even the more restricted Unit-Weight Laplacians can efficiently encode general linear equations over Z_p for smallish p.
Concretely, they give fast algorithms that take a linear equation A x = b (defined by inputs A and b), and return a new equation L y = c, where L is a Laplacian or Unit-Weight Laplacian, such that if one has a solution y to the latter equation, one can quickly obtain a solution x to the original equation.
The Laplacian or Unit-Weight Laplacian equation has size $O(nnz(A))$ or $O(nnz(A)\log^2(p)/\log\log(p))$ respectively (for a natural definition of size).

We can interpret the result as suggesting that it is unlikely that there are fast algorithms for solving (Unit-Weight)Laplacian linear equations over Z_p, or as suggesting that designing such solvers may be a good route for obtaining faster solvers in general for problems over Z_p.

## Strengths
There are at least three good reasons to consider solving (Unit-weight) Laplacian, although these are not that clearly stated by the authors.

(1)
Firstly, as hinted at by the authors, there has been much success in obtaining fast linear equation solvers for Laplacians (and other special matrices) over reals, and it is in itself interesting to know whether one can hope to extend such algorithms to Z_p.

(2)
Secondly, as evidenced by this paper, such an algorithm would turn out to have immediate implications for solving all linear equations over Z_p!

(3)
Thirdly, if a very fast algorithm for solving linear equations over Laplacians in Z_p existed, it would (even without knowing the connection to general linear equations), imply a non-trivially fast algorithm for solving linear equations over Laplacians in Q, an interesting open problem.

The paper establishes a link between the complexity of solving general linear equations over Z_p and (Unit-Weight) Laplacians which is almost as strong as one could possibly hope for.

The observations regarding Unit-Weight Laplacians are quite nice and seem novel.
Firstly, the authors give a very natural definition of the size of a Laplacian matrix represented as a Unit-Weight Laplacian with parallel edges.
Then they use basic facts about series and parallel circuits to show that over Z_p even Unit-Weight Laplacians are very expressive. This surprised me somewhat.

I didn't check the paper carefully beyond the first 10 pages, but the writing seems clear and the arguments easy to follow.

## Weaknesses
In general, the introduction and discussion are quite poor, which I view as particularly problematic given that the STOC audience is not very likely to be familiar with the context of the problem.

Concretely, I think that the potential for impact on solvers over Q should be addressed better.

Also, a connection to the problem studied in [CLL11] is mentioned, but looking at the paper I could not immediately verify that the problem that appears there is equivalent. It would be appropriate to sketch in an appendix why these the linear equations studied there is the same kind of Laplacian.
I would also find it appropriate to cite Dixon's "Exact Solution of Linear Equations Using P-Adic Expansions" or later works on solving rational linear equations using Z_p.

There is no discussion of the state-of-the-art running time for solving linear equations over finite fields (conjugate gradient works!).
This at least deserves a mention. -> fixed by introduction 

The paper is not able to reduce dense linear equations to dense Laplacian linear equations. But this seems to also be a problem in [KZ20], and it doesn't seem too damning as Laplacian linear equation solvers over reals have nearly-linear running time in nnz(L).

The reduction that shows Laplacian linear equations are as hard as general linear equations over Z_p is very simple, bordering on trivial. It makes it look like a Weighted Laplacian is a broken notion over finite fields. On the other hand, that's not really the authors' fault and it seems good to know.

The discussion of the contributions of the authors is somewhat lacking, and in particular, I think it should be mentioned how the general reduction works (I got the feeling this was deliberately omitted) and you might also want to sketch in a couple of sentences how the unit-weight reduction works.

Comments for author
-------------------
```quote
Inversely, these results may also imply unlike over the reals, graph-structured linear systems over the finite field Zp don’t have much special structure information which can help speed up the linear system solvers.
```
- This sentence does not seem to be "inversely" related to the preceding sentence? It seems like there's something missing before this sentence?



To solve Laplacian linear equations over Q it would suffice to solve over Z_p for a random p c.f. Dixon's paper.
Is there a chance that Laplacians over Z_p for random p are easier to solve?
For weighted Laplacians, the answer seems to be no, as your reduction is oblivious to p, but for Unit-Weight Laplacians, it seems less clear. You may want to discuss this.

The role that indices {1,2} play in Definition 10 is not clearly stated and it could potentially be misunderstood by non-experts. You may want to elaborate.

==> stoc22/back_up.tex <==
Proof for Lemma \ref{lem:commutative}
\begin{proof}
    %\todo{add proof}
    Let $S_2 = [n] \setminus T_2$, $S_1 = T_2 \setminus T_1$, $\mL$ can be written as
    \begin{align*}
        \left[
        \begin{array}{ccc}
           \mL_{T_1, T_1} & \mL_{T_1, S_1} & \mL_{T_1, S_2} \\
           \mL_{S_1, T_1} & \mL_{S_1, S_1} & \mL_{S_1, S_2}\\ 
           \mL_{S_2, T_1} & \mL_{S_2, S_1} & \mL_{S_2, S_2}\\ 
        \end{array}
        \right]
    \end{align*}
    and 
    \begin{align*}
        \sc(\mL, T_2) = 
        \left[
        \begin{array}{cc}
           \mL_{T_1, T_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1} &  \mL_{T_1, S_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, S_1} \\
            \mL_{S_1, T_1} - \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1} &  \mL_{S_1, S_1} - \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, S_1} 
        \end{array}
        \right]
    \end{align*}
    Then let $\mC = \sc(\mL_{[[n] \setminus T_1, [n] \setminus T_1]}, S_1) = \mL_{S_1, S_1} - \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, S_1} $, we have
    \begin{align*}
        \sc(\sc(\mL, T_2), T_1) &=  \mL_{T_1, T_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1}  \\ 
        & -(\mL_{T_1, S_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, S_1}) \mC^{-1} (\mL_{S_1, T_1} - \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1})
    \end{align*}
    which equals to 
    \begin{align*}
        \sc(\mL, T_1) &=
        \mL_{T_1, T_1} - 
        \left[
            \begin{array}{cc}
                \mL_{T_1, S_1} & \mL_{T_1, S_2} \\
            \end{array}
        \right]
        \left[
            \begin{array}{cc}
                \mL_{S_1, S_1} & \mL_{S_1, S_2}\\ 
                \mL_{S_2, S_1} & \mL_{S_2, S_2}\\ 
            \end{array}
        \right]^{-1}
        \left[
            \begin{array}{c}
                \mL_{S_1, T_1} \\ 
                \mL_{S_2, T_1}  
            \end{array}
        \right] \\
        &= \mL_{T_1, T_1} - 
        \left[
            \begin{array}{cc}
                \mL_{T_1, S_1} & \mL_{T_1, S_2} \\
            \end{array}
        \right]
        \\
        &
        \quad 
        \left[
            \begin{array}{cc}
                \mC^{-1} & -\mC^{-1} \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1}\\  
                -\mL_{S_2,S_2}^{-1} \mL_{S_2,S_1} \mC^{-1} &  \mL_{S_2,S_2}^{-1} + \mL_{S_2,S_2}^{-1} \mL_{S_2,S_1} \mC^{-1}\mL_{S_1, S_2} \mL_{S_2,S_2}^{-1}
            \end{array}
        \right]
        \left[
            \begin{array}{c}
                \mL_{S_1, T_1} \\ 
                \mL_{S_2, T_1}  
            \end{array}
        \right] \\
        &=  \mL_{T_1, T_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1}  \\ 
        & -(\mL_{T_1, S_1} - \mL_{T_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, S_1}) \mC^{-1} (\mL_{S_1, T_1} - \mL_{S_1, S_2} \mL_{S_2,S_2}^{-1} \mL_{S_2, T_1})
    \end{align*}
    Therefore $\sc(\sc(\mL, T_2), T_1) = \sc(\mL, T_1)$.
\end{proof}


==> stoc22/p13.tex <==
In this section, we show that the class of Laplacian matrices $LS_{\mathbb{Z}_p}$ is efficiently and decisional $f$-reducible to itself for some $f$ that does not depend on the original $\size$ of the matrix. Specifically, the reduction is by replacing every edge in a Laplacian system in $LS_{\mathbb{Z}_p}$ by $\bound$ unit-weight edges. 
\begin{theorem}
\label{thm:p13}
Let $f(\nnz, \size) = (O(\nnz \log^2 p /\log \log p), O(\nnz \log^2 p /\log \log p))$. Then $LS_{\mathbb{Z}_p}\le_fLS_{\mathbb{Z}_p}$.
\end{theorem}
\begin{proof}
We first prove that given any Laplacian system $\mL \in \mathbb{Z}_p^{n\times n}$, we can compute a unit weight Laplacian system $\bar{\mL} \in \mathbb{Z}_p^{k\times k}$ such that 
\begin{enumerate}
    \item $\size(\bar{\mL})\le O(\nnz(\mL)\log^2 p/\log \log p)$.
    \item For any linear system $\mL \vx = \vb$, $\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\bar{\mL} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}$.
\end{enumerate}

Then we will let $\mathcal{A}_{1\mapsto2}(\mL, \vb)=\left(\bar{\mL}, \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right)$, $\mathcal{A}_{2\mapsto1}(\mY)=\{\vy_{[n]}|y\in \mY\}$ and prove their running times.

\paragraph{Construction of $\bar{\mL}$.} We apply Lemma \ref{lem:replace_edge} repeatedly. We let $\mL^{(0)}$ be $\mL$. We fix $n$ as the number of rows in $\mL^{(0)}$. $\mL^{(k)}$ is defined recursively:
\begin{enumerate}
    \item If $\mL^{(k-1)}_{i, j}$ is not $0$ for some $1\le i< j\le n$ satisfying $\forall 1\le \ell < k, (i, j)\neq (i(\ell), j(\ell))$, apply Lemma \ref{lem:replace_edge} for $\mL=\mL^{(k-1)}$, $i_0=i, j_0=j$. Let Lemma \ref{lem:resistance_construction} constructs the circuit $\mR$ in Lemma \ref{lem:replace_edge} with size $\bound$ and resistance $-\mL^{(k-1)}_{i, j}$. Let the resulting $\mU$ be $\mL^{(k)}$. We record the indices $i$ and $j$ as $i(k)$ and $j(k)$. 
    \item Otherwise, $\mL^{(k)}$ is undefined. 
\end{enumerate}
Let $\bar{\mL}$ be $\mL^{(\bar{k})}$ where $\bar{k}$ is the largest $k$ such that $\mL^{(k)}$ is defined. We have $\{(i(1), j(1)), \ldots, (i(\bar{k}), j(\bar{k}))\}$ include every entry of $\mL$ which is strictly above the diagonal and is not equal to $0$ or $p-1$ exactly once. Thus, \begin{equation}
    \size(\mL)\le \nnz(\mL)+\sum_{k=1}^{\bar{k}} 2\left|\mL^{(k-1)}_{i(k), j(k)}\right|\label{eq:sum_of_abs}
\end{equation} and $$\bar{k}\le \nnz(\mL).$$ By Item \ref{itm:replaceitem1} of Lemma \ref{lem:replace_edge},
\begin{align*}
    &\opsize(\bar{\mL})\\
    \le& \opsize(\mL)+\sum_{k=1}^{\bar{k}}\left( -2\left|\mL^{(k-1)}_{i(k), j(k)}\right|+\bound\right)\\
    =& \opsize(\mL)+\sum_{k=1}^{\bar{k}} \left(-2|\mL_{i(k), j(k)}|+\bound\right)\tag{entry $(i(k), j(k))$ is never modified before $\mL^{(k)}$}\\
    =& \opsize(\mL)+\nnz(\mL)-\opsize(\mL)+\sum_{k=1}^{\bar{k}} \bound \tag{by Equation \ref{eq:sum_of_abs}}\\
    \le & O\left(\nnz(\mL)\log^2p/\log\log p\right).\\
\end{align*}
Since $\nnz(\bar{\mL})\le \size(\bar{\mL})$, we have $\nnz(\bar{\mL})=\nnzbound$.

%\paragraph{Proof for $\mathcal{S}\left(\bar{\mL}, \left[\begin{array}{c}\vb \\ 0\end{array}\right]\right)\le f(\mathcal{S}(\mL, \vb))$.} 
Next we prove that for any linear system $\mL \vx = \vb$, $\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\bar{\mL} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}$ by induction. Fix any vector $\vb$. Suppose 
\[\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\mL^{(k)} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}.
\] By Lemma~\ref{lem:replace_edge}, 
\[
\left\{\vy\mid\mL^{(k)} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}\\
    =\left\{\vz_{[\norm{y}_0]}\mid\mL^{(k+1)} \vz = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}
\] where $\norm{\vy}_0$ is the number of coordinates of $\vy$.
Thus,
\begin{align*}
    &\left\{\vx\mid \mL \vx = \vb\right\}\\
    =&\left\{\vy_{[n]}\mid\mL^{(k)} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}\\
    =&\left\{\vz_{[n]}\mid\mL^{(k+1)} \vz = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}.
\end{align*}
By induction, we have 
\[\left\{\vx\mid \mL \vx = \vb\right\} = 
\left\{\vy_{[n]}\mid\mL^{(\bar{k})} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}
=\left\{\vy_{[n]}\mid\bar{\mL} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}.
\]

\paragraph{Running time of $\mathcal{A}_{1\mapsto2}$ and $\mathcal{A}_{2\mapsto1}$.}

$\mathcal{A}_{1\mapsto2}$ simply replaces each non-diagonal non-zero entry by a matrix $\mU$ with $\nnz(\mU)=O(\log^2 p/\log \log p)$. This costs \begin{equation*}
O(\nnz(\bar{\mL}))=O(\nnz(\mL)\log^2 p/\log \log p).
\end{equation*}
We can implement $\mathcal{A}_{2\mapsto1}$ as 
\[
\mathcal{A}_{2\mapsto1}(\vy^*)=(\vy^*_{[n]}).
\] It costs nearly linear time as we only truncate vectors.
\end{proof}
\begin{corollary}
\label{cor:p13}
Let $f(\nnz, \size) = (O(\nnz \log^2 p /\log \log p), O(\nnz \log^2 p /\log \log p))$. Then $LS_{\mathbb{Z}_p}$ is decisional $f$-reducible to $LS_{\mathbb{Z}_p}$.
\end{corollary}
\begin{proof}
    We may use the same $\mathcal{A}_{1\mapsto2}$ as in Theorem \ref{thm:p13}. The algorithm runs in the same time and satisfies 
    \[\mathcal{S}(\mathcal{A}_{1\mapsto2}(\mL,\vb)) \le f(\mathcal{S}(\mL,\vb)).\]
    
    If $\mathcal{A}_{1\mapsto2}(\mL,\vb)$ has a solution $\vy$, $(\mL, \vb)$ has a solution $\vy_{[n]}$. If $(\mL, \vb)$ has a solution $\vx$, $\mathcal{A}_{1\mapsto2}(\mL,\vb)$ must have a solution $\vy$ because otherwise \[\left\{\vx\mid \mL \vx = \vb\right\}\neq \emptyset=\left\{\vy_{[n]}\mid\bar{\mL} \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}.\] Thus, the outputs to $\mathcal{A}_{1\mapsto2}(\mL,\vb)$ and to $(\mL,\vb)$ are always the same.
\end{proof}
\subsubsection{Construction of size-$\bound$ circuit}
In this section, we construct a circuit over $\mathbb{Z}_p$ with any resistance in $[1, p-1]$ within $\bound$ size. We will say the resistance $r$ of a circuit $\mL$ is equivalent to $w$ for any $w\in \mathbb{Z}$ such that $r\equiv w\pmod p$. 
\begin{lemma}
\label{lem:resistance_construction}
Let $r$ be an integer in $[1, p-1]$. There exists a circuit with size $\bound$ and resistance $r$.
\end{lemma}
To construct any resistance value, we first need the following three lemmas which construct any resistance of the form $ab^{-1}$ within size $O(a+b)$. 
\begin{lemma}
\label{lem:z}
Given two circuits with resistances $1$ and $z$ and sizes $n$ and $m$ respectively, we can construct the following circuits:
\begin{itemize}
    \item A circuit with resistance $1+z$ and size $n+m$.
    \item A circuit with resistance $z(z+1)^{-1}$ and size $n+m$.
\end{itemize}
\end{lemma}
\begin{proof}
Let these two circuits be $\mL$ and $\mU$. By Lemma \ref{lem:pa_and_se}, $\series(\mL, \mU)$ has resistance $1+z$ and size $n+m$. $\parallel(\mL, \mU)$ has resistance $z(z+1)^{-1}$ and size $n+m$. 
\end{proof}
\begin{lemma}
\label{lem:onestep}
By two circuits with resistances $1$ and $ab^{-1}$ and sizes $n$ and $m$, we can construct the following circuits:
\begin{itemize}
    \item A circuit of resistance $(a+b)b^{-1}$  and size $n+m$.
    \item A circuit of resistance $a(a+b)^{-1}$ and size $n+m$.
\end{itemize}
\end{lemma}
\begin{proof}
By Lemma \ref{lem:z} with $z=ab^{-1}$.
\end{proof}
\begin{lemma}
\label{lemma:sqrtconstruction}
We can construct a circuit of size $O(M)$ and resistance equivalent to $ab^{-1} \bmod p$ for any $a, b\in \mathbb{Z}$ such that $1\le a, b\le M$.
\end{lemma}
\begin{proof}
We construct the value $ab^{-1} \bmod p$ recursively. If $a>b$, we can construct $ab^{-1} \bmod p$ from $(a-b)b^{-1} \bmod p$ and another unit circuit by Lemma \ref{lem:onestep}. If $a<b$, we can construct $ab^{-1} \bmod p$ from $a(b-a)^{-1} \bmod p$ and another unit circuit by Lemma \ref{lem:onestep}. If $a=b$, we can construct $ab^{-1}\equiv 1 \pmod p$ by just one unit circuit. Since $a, b$ are always positive integers and their initial values are no more than $M$ in $\mathbb{Z}$, this process ends in $O(M)$ steps.
\end{proof}
Then we are able to construct resistance values near $\frac{pi}{j}$ (one of the points that exactly divide $[1, p-1]$ into $j$ equal parts).
\begin{lemma}
\label{lem:fracK}
Let $k\in \mathbb{Z}$ be an integer in $[1, p-1]$. For any $1\le i\le j\le k$, there exists a circuit $\mL$ with size $O(k)$ and resistance equivalent to some integer $w\in [\frac{pi}{j}, \frac{pi}{j}+1]$.
\end{lemma}
\begin{proof}
Let $w = \lceil pi/j \rceil \in \mathbb{Z}$. It follows that $w \in [\frac{pi}{j}, \frac{pi}{j}+1]$. Now $w = \frac{\lceil pi/j \rceil j}{j}$ as integers, and thus $w \equiv (\lceil pi/j \rceil j)j^{-1} \bmod p$. Now $pi \leq \lceil pi/j \rceil j \leq pi+j$, so $(\lceil pi/j \rceil j) \bmod p \leq j$. By Lemma \ref{lemma:sqrtconstruction}, we can construct a circuit with resistance $w \bmod p$ and size $O(j) = O(k)$.
\end{proof}


Since $-x\equiv p-x \pmod p$, we can also construct resistance values near $-\frac{pi}{j}$ for some $0\le i\le j$.
\begin{corollary}
\label{cor:fracK}
Let $k\in \mathbb{Z}$ be an integer in $[1, p-1]$. For any $1\le j\le k$ and $-j\le i\le j$, there exists a circuit $\mL$ with size $O(k)$ and resistance equivalent to some integer $w\in [\frac{pi}{j}, \frac{pi}{j}+1]$.
\end{corollary}
\begin{proof}
When $i$ is $0$, we let $\mL$ be the unit circuit. When $i$ is positive, this is equivalent to Lemma \ref{lem:fracK}. When $i$ is negative, we first construct a circuit $\mL$ with size $O(k)$ and resistance equivalent to $\bar{w}$ for some $\bar{w}\in [p(j+i)/j, p(j+i)/j+1]$ by Lemma \ref{lem:fracK}. Then the resistance of $\mL$ is also equivalent to $w$ for $w=\bar{w}-p\in [pi/j, pi/j+1]$ because $w\equiv \bar{w}-p \pmod p$.
\end{proof}
%\begin{lemma}
%\label{lem:fracK2}
%Let $k$ be an integer in $[1, p-1]$. For any $1\le i\le k(k-1)$, there exists an electric circuit with size $O(k)$ unit resistors and resistance $r\in [\frac{pi}{k(k-1)}, \frac{pi}{k(k-1)}+4]$.
%\end{lemma}
%\begin{proof}
%By the Extended Euclidean algorithm, we know $\frac{i}{k(k-1)}=\frac{a}{k}+\frac{b}{k-1}$ for some integer $a\in [-k, k]$ and $b$ in $[-(k-1), k-1]$.

%We construct two circuits $\mL$ and $\mU$ with resistances equal to $x$ in $[ap/k, ap/k+2]$ and $y$ in $[bp/(k-1), bp/(k-1)+2]$ respectively by Corollary \ref{cor:fracK}. Both of them are of size $O(k)$. 

%By Lemma \ref{lem:pa_and_se}, $\series(\mL, \mU)$ has resistance $x+y\in [i p / (k^2-k), i p / (k^2-k)+4]$ and size $O(k)$.
%\end{proof}
By adding the resistances given by Corollary \ref{cor:fracK} for several different prime numbers $j_1, \ldots, j_t$, we can construct resistances near $\frac{pi}{j}$ for $j=\prod_{s=1}^t j_s$ and any $-j\le i\le j$.
\begin{lemma}
\label{lem:fracK2}
Let $k\in \mathbb{Z}$ be an integer in $[1, p-1]$. Let $j_1< \ldots< j_t$ be $t$ different primes in $[1, k]$. For any $-j\le i\le j$ for $j\defeq \prod_{s=1}^t j_s$, there exists an integer $w$ and an electric circuit with size $O(kt)$ and resistance equivalent to some integer $w\in [\frac{pi}{j}, \frac{pi}{j}+2t]$.
\end{lemma}
\begin{proof}
We first write $\frac{i}{j}$ as $\sum_{s=1}^t \frac{a_s}{j_s}$ for some $a_1,\ldots, a_t$ satisfying $\forall 1\le s\le t, a_s\in [-j_s, j_s]$. 

$a_1,\ldots, a_t$ can be found recursively. We first find an $a_t$ such that 
\begin{enumerate}
    \item \label{itm:cdt1} $\frac{i}{j}-\frac{a_t}{j_t}=\frac{\bar{i}}{j/j_t}$ for some integer $\bar{i}$, and 
    \item \label{itm:cdt2} $-j/j_t\le \bar{i} \le j/j_t$.
\end{enumerate} We let 
\[
a_t=\left(i(j/j_t)^{-1}\right)\bmod {j_t}
\] where $(j/j_t)^{-1}$ is the inverse of $j/j_t$ modulo ${j_t}$. The inverse exists since $j/j_t$ is the product of primes less than $j_t$. Then Condition \ref{itm:cdt1} is satisfied. Because 
\[-1\le\frac{i}{j}\le 1\text{ and }-1\le -\frac{a_t}{j_t}\le 0,\]
we have \[\frac{\bar{i}}{j/j_t}\le 1.\] 
If 
\[\frac{i}{j}-\frac{a_t}{j_t}\ge -1,\]
Condition \ref{itm:cdt2} is also satisfied. 
Otherwise, 
\[-2\le \frac{i}{j}-\frac{a_t}{j_t}< -1.\] 
In this case, we decrease $a_t$ by $j_t$ and $\bar{i}$ by $j/j_t$ to fulfill Condition \ref{itm:cdt2}. 
Condition \ref{itm:cdt1} still holds because both sides of the equation increase by $1$.

$a_{t-1},\ldots, a_1$ can be constructed recursively by \[\frac{\bar{i}}{j/j_t}=\sum_{s=1}^{t-1} \frac{a_s}{j_s}.\]

After deciding $a_1,\ldots, a_t$, we construct $t$ size-$O(k)$ circuits $\mL_1,\ldots, \mL_t$ such that $\mL_s$ has resistance that is equivalent to some integer in 
\[[pa_s/j_s, pa_s/j_s+2]\] by Corollary \ref{cor:fracK}. Then 
\[\series(\mL_1, \series(\mL_2, \ldots, \series(\mL_{t-1}, \mL_t)\ldots))\] has size $O(tk)$ and resistance $r$ equivalent to some integer $w$ between $[\frac{pi}{j}, \frac{pi}{j}+2t]$.
\end{proof}
Lemma \ref{lem:fracK2} can construct any resistance between $[1, p-1]$ up to a small additive error. We prove Lemma \ref{lem:resistance_construction} by fixing the error.
\begin{proof}[Proof for Lemma \ref{lem:resistance_construction}]
    Let $t$ be the smallest integer such that $p\le \prod_{s=1}^t j_s$, where $j_s$ is the $s$-th smallest prime. Let $j=\prod_{s=1}^t j_s$. Let $k=j_t$. We can construct a size-$O(tk)$ circuit $\mL_i$ with resistance equivalent to $x_i$ in $[\frac{pi}{j}, \frac{pi}{j}+2t]$ for any $i\in [1, j]$ by Lemma \ref{lem:fracK2}. Since $j\ge p$, we know $|x_{i+1}-x_i|\le 1+2t$. Let 
    \[X=\{x_0\defeq 0, x_1, \ldots, x_{j}, x_{j+1}\defeq p\}.\]
    Since $|x_{i+1}-x_i|=O(t)$ for any $1\le i<j$, $x_1=O(t)$ and $|p-x_{j}|=O(t)$, any number $z$ in $[1, p-1]$ must be between $x_i$ and $x_{i+1}$ for some $0\le i\le j$. Thus, $z$ can be written as the sum of some $x_i\in X$ and some other non-negative integer $y=O(t)$. (In other words, $z=\min(x_i, x_{i+1})+y$.) Let $\mU_y$ be a circuit with resistance equivalent to $y$ and size $O(y)$. ($\mU_y$ can be a path of length $y$.) If $i=0$, $\mU_y$ is the desired circuit. If $i>0$, by Lemma \ref{lem:pa_and_se}, $\series(\mL_i, \mU_y)$ is a circuit with resistance equivalent to $z$ and size $O(kt)$. By the Prime Number Theorem \cite{P1896, H1896}, we can show that $t \le \log p/\log\log p$ and $k=p_t\le \log p$. Thus, $O(kt)=\bound$.
\end{proof}

We can show our construction of circuits with given resistance modulo $p$ can be implemented efficiently:

\begin{lemma}
\label{lem:complexity}
Using the constructions   is possible to construct a circuit $\mU$ with resistance $z \in [p-1]$ in $O(\log^3 p)$ time.
\end{lemma}

\begin{proof}
Given $\mL \in \mathbb{Z}^{n \times n}_p$ and $\mU \in \mathbb{Z}^{m \times m}_p$, the construction of $\parallel(\mL,\mU)$ and $\series(\mL,\mU)$ in Lemma \ref{lem:pa_and_se} can be done in $O(\nnz(\mL) + \nnz(\mU)) = O(\size(\mL) + \size(\mU))$ time because $\parallel(\mL,\mU)$ and $\series(\mL,\mU)$ can be obtained by re-arranging the non-zero entries of $\mL$ and $\mU$ plus performaing a constant number of additions. As a result, the construction in Lemma \ref{lem:z} can be done in $O(n+m)$ time given two circuits with resistances 1 and $z$ and sizes $n$ and $m$. The construction in Lemma \ref{lem:onestep} can be done in $O(n+m)$ time given two circuits with resistances 1 and $ab^{-1}$ and sizes $n$ and $m$. 

In Lemma \ref{lemma:sqrtconstruction}, suppose we are given $a,b \in [M]$, we can construct a circuit with resistance $ab^{-1} \mod p$ in at most $M$ steps and each step involves connecting a unit circuit with the circuit constructed by recursing on $(a-b)b^{-1} \bmod p$ or $a(b-a)^{-1} \bmod p$. Therefore, the construction in Lemma \ref{lemma:sqrtconstruction} can be completed in $O(M^2)$ time. As a result, given $i \leq j, i,j \in [k]$, we can construct a circuit $\mL$ with resistance equivalent to some integer $w \in [\frac{pi}{j}, \frac{pi}{j}+2]$ in $O(k^2)$ time. By Corollary \ref{cor:fracK}, given $k \in [p-1]$, for any $i,j \in [k]$, $-j \leq i \leq j$, we can construct a circuit $\mL$ with resistance equivalent to some integer $w \in [\frac{pi}{j}, \frac{pi}{j}+2]$ in $O(k^2)$ time.

Now we may analyze the runtime for the construction done by Lemma \ref{lem:fracK2}. We may find the $a_t$s in $O(t)$ time and construct circuits $\mL_1,\ldots,\mL_t$ with resistance equivalent to some integer in $[pa_s/j_s,pa_s/j_s+2]$ in $O(tk^2)$ time and connect them in serial in $O(t^2k)$ time. This results in a complexity of $O(tk^2) + O(t^2k) = O(tk(k+t))$.

Finally, we examine the construction in Lemma \ref{lem:resistance_construction}. Finding the smallest integer $t$ such that $p \leq \prod_{s=1}^t j_s$ can be done in $O(\log^2 p)$ time since $j_t \leq \log p$. $x_i = \sum_{s=1}^t \lceil \frac{pa_s}{j_s} \rceil$  can be computed exactly in $O(t)$ time for a given $i$. Since $x_0 = 0 < z$, $x_{j+1} := p > z$, we can use divide-and-conquer to find an $i$ such that $z$ is between $x_i$ and $x_{i+1}$ in $O(\log j) = O(\log (kp))$ steps, so we can find the $i$ and write $z$ as $z = \min(x_i,x_{i+1})+y$ in $O(\log(kp)t) = O(\log^2 p)$ time. Since $\mU_y$ is just a path of length $y$, we can construct $\mU_y$ in $O(y^2) = O(t^2)$ time, and by our analysis for Lemma 4.11, $\mL_i$ can be constructed in $O(tk(t+k))$ time. Next, connect $\mL_i$ and $\mU_y$ in serial should be done in $O(tk)$ time since $\size(\mL_i) = O(tk)$ and $\size(\mU_y) = O(t)$. As a result, given the bounds $t \leq \log p/\log \log p$ and $t \leq \log p$, we can construct the final circuit $\mU$ in $O(\log^3p)$ time.

\end{proof}



==> stoc22/preamble.tex <==
\textheight 8.5in
\topmargin -0.2in
\oddsidemargin 0.20in
\textwidth 6.3in
%\oddsidemargin -0.5in
%\evensidemargin -0.5in
%\textwidth 7.2in
%\topmargin -0.5in
%\textheight 8in
\flushbottom

\usepackage[colorlinks=true,linkcolor=blue,citecolor=blue]{hyperref}
\usepackage{bm}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{cite}
\usepackage{makecell}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{fancybox}
\usepackage{multirow}
\usepackage{tikz}

%% Theorems
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{fact}{Fact}
\newtheorem*{lemma*}{Lemma}

%% Linear Algebra
\newcommand{\tran}[0]{\ensuremath{^{\mathsf{T}}}\xspace}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\providecommand{\eye}{\ensuremath{\mat{I}}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mSigma}{\ensuremath{\mat{\Sigma}}}
\providecommand{\vone}{\ensuremath{\vec{1}}}
\providecommand{\vzero}{\ensuremath{\vec{0}}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{l}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}
\providecommand{\vchi}{\ensuremath{\vec{\chi}}}
\providecommand{\vpi}{\ensuremath{\vec{\pi}}}
\providecommand{\vlambda}{\ensuremath{\vec{\lambda}}}
\providecommand{\vepsilon}{\ensuremath{\vec{\epsilon}}}
\newcommand{\norm}[1]{\left\lVert #1\right\rVert}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}

\renewcommand{\bar}[1]{\overline{#1}}
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\newcommand*{\defequiv}{\stackrel{\text{def}}{\equiv}}
\newcommand{\Otil}{\widetilde{O}}
\def\polylog{\operatorname{polylog}}
\newcommand{\bound}{O\left(\log^2p/\log\log p\right)}
\newcommand{\nnzbound}{O\left(\nnz(\mA)\log^2p/\log\log p\right)}
\newcommand{\lscp}{SLS}
\newcommand{\lsdp}{DPLS}
\newcommand{\GS}{\ensuremath{\mathcal{GS}}}
\newcommand{\LS}{\ensuremath{\mathcal{LS}}}
%\renewcommand{\parallel}{\mathrm{para}}
%\newcommand{\series}{\mathrm{seri}}
\renewcommand{\parallel}{\textsc{Para}}
\newcommand{\series}{\textsc{Seri}}
\newcommand{\size}{\mathrm{size}}
% fix spacing in align*, use this as an operator
\DeclareMathOperator{\opsize}{size}
\newcommand{\nnz}{\mathrm{nnz}}
\renewcommand{\sc}{\mathbf{SC}}

%%comments
\newcommand{\rp}[1]{\textbf{\color{blue} Richard: #1}}
\newcommand{\yh}[1]{\textbf{\color{green} Yufan: #1}}
\newcommand{\gy}[1]{\textbf{\color{yellow} Yu: #1}}
\newcommand{\jb}[1]{\textbf{\color{green} Jingbang: #1}}
\newcommand{\rw}[1]{\textbf{\color{purple} Runze: #1}}
\newcommand{\todo}[1]{{\textbf{\color{red} TODO: #1}}}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

==> stoc22/reductiontolaplacian.tex <==
In this section we show that the class of general matrices $\GS_{\mathbb{Z}_p}$ is efficiently and decisional $f$-reducible to the class of Laplacian matrices $\LS_{\mathbb{Z}_p}$ for specifically chosen $f$.
\begin{theorem}
\label{theorem_GfL}
      Let $f(\nnz, \size) = (O(\nnz), O(\nnz \times p))$, then $\GS_{\mathbb{Z}_p} \le_{f} \LS_{\mathbb{Z}_p}$.
\end{theorem} 

\begin{proof}
\ We first prove that given any linear system $(\mA \in \mathbb{Z}_p^{m \times n}, 
\vb \in \mathbb{Z}_p^{m}) \in \GS_{\mathbb{Z}_p}$, we can compute a Laplacian system 
$(\mL \in \mathbb{Z}_p^{2(m+n) \times 2(m+n)}, \vc \in \mathbb{Z}_p^{2(m+n)})$ such 
that 

\begin{enumerate}
    \item $\nnz(\mL) = O(\nnz(\mA))$ 
    \item $\{\vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n} \mid \mL \vy = \vc \} = 
    \{ \vx \mid \mA \vx = \vb \}$
\end{enumerate}

Then we will let $\mathcal{A}_{1 \mapsto 2}(\mA, \vb) = (\mL, \vc)$, $\mathcal{A}_{2 \mapsto 1}(\mL, \vc, \vy) = \vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n}$ and show their running times.


\paragraph{Construction of $(\mL, \vc)$}

Inspired by \cite{KOSZ13}, we construct $(\mL, \vc)$ as 

%\begin{align*}
%     \mathcal{A}_{1 \mapsto 2}(\mA, \vb) &= (\mL \defeq 
%     \left[ 
%            \begin{array}{cccc}
%                \vzero & \mA & \vzero &  -\mA \\
%                \mA^T & \vzero & -\mA^T & \vzero \\
%                \vzero & -\mA & \vzero & \mA \\
%                -\mA^T & \vzero & \mA^T & \vzero
%            \end{array}
%            \right],
%            \vc \defeq  
%            \left[
%            \begin{array}{c}
%            \vb \\
%            \vzero \\
%            -\vb \\
%            \vzero
%            \end{array}
%            \right]
%     )
%\end{align*}
\begin{align*}
     \mL \defeq 
     \left[ 
            \begin{array}{cccc}
                \vzero & \mA & \vzero &  -\mA \\
                \mA^T & \vzero & -\mA^T & \vzero \\
                \vzero & -\mA & \vzero & \mA \\
                -\mA^T & \vzero & \mA^T & \vzero
            \end{array}
            \right],\quad
            \vc \defeq  
            \left[
            \begin{array}{c}
            \vb \\
            \vzero \\
            -\vb \\
            \vzero
            \end{array}
            \right]
\end{align*}
It's easy to verify $\mL$ is symmetric and
    \begin{align*}
        \mL \vone = 
        \left[
        \begin{array}{cccc}
        \vzero & \mA & \vzero & -\mA \\
        \mA^T & \vzero & -\mA^T & \vzero \\
        \vzero & -\mA & \vzero & \mA \\
        -\mA^T & \vzero & \mA^T & \vzero \\ 
        \end{array}
        \right]
        \left[
        \begin{array}{c}
            \vone \\
            \vone \\
            \vone \\
            \vone \\
        \end{array}
        \right]
        = 
        \left[
        \begin{array}{c}
            \mA - \mA \\
            \mA^T - \mA^T \\
            \mA - \mA \\
            \mA^T - \mA^T \\
        \end{array}
        \right]
        = \bm{0}
    \end{align*}
    which implies $\vone$ is in the nullspace of $\mL$. 
    According to Definition \ref{matrix::zp}, $\mL$ is a Laplacian matrix over the finite field $\mathbb{Z}_p$. 
\paragraph{Proof for $\mathcal{S}(\mL, \vc) \le f(\mathcal{S}(\mA, \vb))$}
    By our construction of $\mL$, we have $\nnz(L) = O(\nnz(\mA))$. Besides we have $\mA \in \mathbb{Z}_p^{m \times n}$, thus $\size(L) = O(p \times \nnz(\mA))$. Therefore
    \begin{align*}
        \mathcal{S}(\mL, \vc) \le (O(\nnz(\mA), O(p \times \nnz(\mA))) = f(\mathcal{S}(\mA, \vb)) 
    \end{align*}
%    Besides, the running time of $\mathcal{A}_{1 \mapsto 2}$ is bounded by $O(\nnz(\mA))$.
Next we show $\{\vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n} \mid \mL \vy = \vc \} = 
    \{ \vx \mid \mA \vx = \vb \}$. 
Considering a solution $\vy = (\vy_1^T, \vy_2^T, \vy_3^T, \vy_4^T)^T$ to the linear system $\mL \vy = \vc$ 
%where $\vy_1 = \vy_{[1, m]}, \vy_2 = \vy_{[m+1, m+n]}, \vy_3 = \vy_{[m+n+1, 2m+n]}, \vy_4 = \vy_{[2m+n+1, 2m+2n]} $
, we have
    \begin{align*}
    \left. 
    \begin{array}{r @{{}={}} l}
        \mA \vy_2 - \mA \vy_4 & \vb   \\
        \mA^T \vy_1 - \mA^T \vy_3 & \vzero   \\
        -\mA \vy_2 + \mA \vy_4 & -\vb   \\
        -\mA^T\vy_1 + \mA^T \vy_3 & \vzero   \\
    \end{array}
    \right\}
    \text{ implies } \mA(\vy_2 - \vy_4) = \vb  
    \end{align*}
     Thus 
     \begin{align*}
        \vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n} = \vy_2 - \vy_4 \in \{ \vx \mid \mA \vx = \vb   \} 
     \end{align*}
     For every solution $\vx$ to $\mA \vx = \vb  $, we have
     \begin{align*}
        \left[
        \begin{array}{cccc}
        \vzero & \mA & \vzero & -\mA \\
        \mA^T & \vzero & -\mA^T & \vzero \\
        \vzero & -\mA & \vzero & \mA \\
        -\mA^T & \vzero & \mA^T & \vzero \\ 
        \end{array}
        \right]
        \left[
        \begin{array}{c}
            \vzero \\
            \vx \\
            \vzero \\
            \vzero \\
        \end{array}
        \right]
        = 
        \left[
        \begin{array}{c}
            \mA \vx \\
            \vzero \\
            -\mA \vx \\
            \vzero \\
        \end{array}
        \right]
        = 
        \left[
        \begin{array}{c}
            \vb \\
            \vzero \\
            -\vb \\
            \vzero \\
        \end{array}
        \right]
        = \vc  
 \end{align*}
which implies
\begin{align*}
    \vy = \left[
        \begin{array}{c}
            \vzero \\
            \vx \\
            \vzero \\
            \vzero \\
        \end{array}
        \right]
\end{align*}
is a solution to the linear system $\mL \vy = \vc  $. Since $\vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n} = \vx - \vzero = \vx$,
\begin{align*}
    \vx \in\{\vy_{m+1:m+n} - \vy_{2m + n + 1:2m + 2n} \mid \mL \vy = \vc \}
\end{align*}
\paragraph{Running time of $\mathcal{A}_{2 \mapsto 1}$, $\mathcal{A}_{1 \mapsto 2}$}

By our construction of $(\mL, \vc)$, we have $\mathcal{A}_{1 \mapsto 2}$ run in $O(\nnz(\mA))$ time. Since $\vx = \vy_{[m+1, m+n]} - \vy_{[2m + n + 1, 2m + 2n]}$,
$\mathcal{A}_{2 \mapsto 1}$ runs in $O(n) = O(\nnz(\mA))$ time.
%
%For the solution space $\mX = \begin{bmatrix}{\vx^*, \vv_1, \vv_2 \ldots, \vv_r}\end{bmatrix}$
%of the LSCP instance $(\mL, \vc)$ where
%\begin{align*}
%    (\mL, \vc) = \mathcal{A}_{1 \mapsto 2}(\mA, \vb)
%\end{align*}
%we construct $\mathcal{A}_{2 \mapsto 1}$ as
%\begin{align*}
%   \mathcal{A}_{2 \mapsto 1}(\mL, \vc, \mX) = 
%   \begin{bmatrix}
%        \vx^*_{S} - \vx^*_{T}, (\vv_1)_S - (\vv_1)_T, \ldots, (\vv_r)_S - (\vv_r)_T  
%   \end{bmatrix}
%\end{align*}
%where $S = [n+1, 2n], T = [3n+1, 4n]$. Notice that $\mathcal{A}_{2 \mapsto 1}$ runs in $O(\nnz(\mX))$ time as we operate each non-zero entry of $\mX$ at most once.
%
%\begin{lemma}
%    $\mathcal{A}_{2 \mapsto 1}(\mL, \vc, \mX)$ returns the solution space of the LSCP instance $(\mA, \vb)$.
%\end{lemma}
%\begin{proof}
%    To prove this, we only needs to show that 
%    \begin{align*}
%        \mA(\vx_S^* - \vx_T^*) = \vb   
%    \end{align*}
%    and $(\vv_1)_S - (\vv_1)_T, \ldots, (\vv_r)_S - (\vv_r)_T$ spans the nullspace of
%    $\mA$, i.e. 
%    \begin{align*}
%        \{ \sum_{i=1}^r \vc_i \left((\vv_i)_S - (\vv_i)_T \right) \mid \vc \in \mathbb{Z}_p^{r}\} = \{ \vx \mid \mA \vx = \vzero  \}
%    \end{align*}
%    By Lemma \ref{solution_space_lemma}, we know it's equivalent to prove
%    \begin{align*}
%        \{ \sum_{i=1}^r \vc_i \left((\vv_i)_S - (\vv_i)_T \right) \mid \vc \in \mathbb{Z}_p^{r}\} = \{ \vy_S - \vy _T \mid \mL \vy = \vc   \} 
%    \end{align*}
%    First as $\vx^*$ is a solution to $\mL \vy = \vc  $, we know
%    \begin{align*}
%        \mA \vx^*_S - \mA \vx^*_T = \vb    
%    \end{align*}
%    Second by definition of $\mX$, we know 
%    \begin{align*}
%        & \quad \{ \sum_{i=1}^r \vc_i \vv_i \mid \vc \in \mathbb{Z}_p^r \} = 
%        \{ \vy \mid \mL \vy = \vc   \} \\
%        & \Rightarrow  \{ (\sum_{i=1}^r \vc_i \vv_i)_S - (\sum_{i=1}^r \vc_i \vv_i)_T \mid \vc \in \mathbb{Z}_p^r \} = 
%        \{ \vy_S - \vy_T \mid \mL \vy = \vc   \} \\
%        & \Rightarrow  \{ \sum_{i=1}^r \vc_i \left((\vv_i)_S - (\vv_i)_T \right) \mid \vc \in \mathbb{Z}_p^{r}\} = \{ \vy_S - \vy _T \mid \mL \vy = \vc   \} 
%    \end{align*}
%\end{proof}
%
%\yufan{need to fill this proof}
\end{proof}
\begin{corollary}
\label{cor:GFL}
      Let $f(\nnz, \size) = (O(\nnz), O(\nnz \times p))$, then $GS_{\mathbb{Z}_p}$ is decisional $f$-reducible to $LS_{\mathbb{Z}_p}$.
\end{corollary} 
\begin{proof}
We may use the same $\mathcal{A}_{1 \mapsto 2}$ as in Theorem \ref{theorem_GfL}. The algorithm runs in the same time and satisfies
\begin{align*}
    \mathcal{S}(\mathcal{A}_{1 \mapsto 2}(\mA, \vb)) \le f(\mathcal{S}(\mA, \vb))
\end{align*}
If $\mathcal{A}_{1 \mapsto 2}(\mA, \vb)$ has a solution $\vy$, $(\mA, \vb)$ has a solution $\vy_{m+1:m+n} - \vy_{2m+n+1:2m+2n}$. If $(\mA, \vb)$ has a solution $\vx$, $\mathcal{A}_{1 \mapsto 2}(\mA, \vb)$ must have a solution $\vy$ because otherwise
\begin{align*}
    \{ \vx \mid \mA \vx = \vb \} \neq \emptyset = \{ \vy_{m+1:m+n} - \vy_{2m+n+1:2m+2n} \mid \mL \vy = \vc \}
\end{align*}
Thus, the outputs to $\mathcal{A}_{1 \mapsto 2}(\mA, \vb)$ and to $(\mA, \vb)$ are always the same.
\end{proof}

==> stoc22/sec-schur.tex <==
\section{Schur Complement over $\mathbb{Z}_p$}
\label{sec3}

In this section we introduce the definition of Schur complement over $\mathbb{Z}_p$ and its basic properties. We show that just constructing
these objects suffices for carrying out
reductions between linear systems classes.

\begin{definition}
    For any square matrix $\mA \in \mathbb{Z}_p^{n \times n}$, let $T \subseteq [n]$ be some index set and $S = [n] \setminus T$, then $\mA$ can be written as
    $
    \left[
    \begin{array}{cc}
    \mA_{T,T} & \mA_{T,S} \\
    \mA_{S, T} & \mA_{S, S}
    \end{array}
    \right]
    $ 
    where $\mA_{T, T}, \mA_{T, S}, \mA_{S, T}, \mA_{S, S}$ are block matrices. The Schur complement of $\mA$ with respect to $T$ is defined as    
    \begin{align*}
        \sc(\mA, T) = \mA_{T, T} - \mA_{T, S} \mA_{S, S}^{-1} \mA_{S, T}
    \end{align*}
    which exists when $\mA_{S, S}$ is non-singular.
\end{definition}

\subsection{Reduction by Schur Complement}

The following three lemmas state that the Schur complement always preserves the solution space as it can be seen as doing Gaussian elimination partly in advance. We will use them to prove that we can reduce a Laplacian linear system by replacing an edge with another graph with the same resistance (Lemma \ref{lem:replace_edge}).

\begin{lemma}
\label{lem:sc_preserve_sol_1}
    Let $\vx$ be a solution vector for the linear system 
    $\mA \vx = \left[\begin{array}{c} \vb \\ \vzero \end{array}\right]$, and $T$ be the indices of $\vb$. If $\sc(\mA, T)$ exists, then $\sc(\mA, T) \vx_T = \vb$.  
\end{lemma}
\begin{proof}
    Write $\vx = 
    \left[ 
    \begin{array}{c}
    \vx_T \\
    \vx_S
    \end{array}
    \right]$,
    we have
    \begin{align*}
        \left[
        \begin{array}{cc}
           \mA_{T, T}  & \mA_{T, S} \\
           \mA_{S, T}  & \mA_{S, S} \\
        \end{array}
        \right]
        \left[
        \begin{array}{c}
             \vx_T  \\
             \vx_S  \\
        \end{array}
        \right]
        =
        \left[
        \begin{array}{c}
            \vb  \\
            \vzero  
        \end{array}
        \right]
    \intertext{ which implies }
    \mA_{T, T} \vx_T + \mA_{T, S} (-\mA_{S, S}^{-1} \mA_{S,T} \vx_T) =  \sc(\mA, T)\vx_T =  \vb  
    \end{align*}
    where the existence of $\mA_{S, S}^{-1}$ is guaranteed by the assumption $\sc(A, T)$ exists. 
\end{proof}

\begin{lemma}
\label{lem:sc_preserve_sol_2}
Let $\vx_T$ be a solution vector of $\sc(\mA, T) \vx_T=\vb$. Then there exists an extension $\vx$ of $\vx_T$ such that $\mA \vx=\left[\begin{array}{c}\vb\\ \vzero \end{array}\right]$. 
\end{lemma}

\begin{proof}
   By taking $\vx_S = -\mA_{S, S}^{-1} \mA_{S, T} \vx_T$ and extending $\vx_T$ to 
   $\vx = 
   \left[ 
   \begin{array}{c}
      \vx_T    \\
      \vx_S   
   \end{array}
    \right]$, we have 
    \begin{align*}
        \left[
        \begin{array}{cc}
           \mA_{T, T}  & \mA_{T, S} \\
           \mA_{S, T}  & \mA_{S, S} \\
        \end{array}
        \right]
        \left[
        \begin{array}{c}
             \vx_T  \\
             \vx_S  \\
        \end{array}
        \right]
        = 
        \left[
        \begin{array}{c}
             \mA_{T,T} \vx_T + \mA_{T,S} (-\mA_{S, S}^{-1} \mA_{S, T} \vx_T)  \\
             \mA_{S,T} \vx_T - \mA_{S,S} \mA_{S,S}^{-1} \mA_{S,T} \vx_T  \\
        \end{array}
        \right]
        = 
        \left[
        \begin{array}{c}
            \sc(\mA, T) \vx_T \\
            \vzero
        \end{array}
        \right]
        =
        \left[
        \begin{array}{c}
            \vb \\
            \vzero
        \end{array}
        \right]
    \end{align*}
\end{proof}

A proof for the following Lemma can be found in \cite{OSTROWSKI1971}.
\begin{lemma}
\label{lem:commutative}
Let $\mL\in \mathbb{Z}^{n\times n}_p$ be a Laplacian matrix. Let $T_1\subseteq T_2$ be two subsets of $[n]$. Then $\sc(\mL, T_1)=\sc(\sc(\mL, T_2), T_1)$.
\end{lemma}

In our construction, we will repeatedly identify pairs of nodes in two graphs to combine them into a new graph with some desired property. The following definition of circuit simplifies our presentation. Any Laplacian system in $\mathbb{Z}_p$ can be viewed as a unit-weight Laplacian because an entry $\mL_{i, j}=p-x$ is equivalent to $x$ parallel unit-weight edges. We also define $\size$ below as the number of such edges.
\begin{definition}
\label{def:circuit}
    An Laplacian system $\mL\in \mathbb{Z}^{n\times n}_p$ is called a circuit with weight $r$ (or equivalently resistance $r^{-1}$) if  $\sc(\mL, \{1, 2\})=\vchi_{1, 2}^\top r \vchi_{1, 2}$. The size of $\mL$ is defined as $\sum_{1\le i\neq j \le n} |\mL_{i, j}|$ where $|x|$ for any $x\in \mathbb{Z}_p$ is defined as $(p-x)\bmod p$ as a number in $\mathbb{Z}$.
    We call $\left[\begin{array}{cc} 1 & -1 \\ -1 & 1\end{array}\right]$ the unit circuit.
\end{definition}

\begin{lemma}
\label{lem:replace_edge}
Given any Laplacian system $\mL \in \mathbb{Z}_p^{n\times n}$, a non-zero non-diagonal entry $\mL_{i_0, j_0}$ and a circuit $\mR$ with weight $-\mL_{i_0, j_0}$ and size $s$, we can compute a Laplacian system $\mU \in \mathbb{Z}_p^{(n+m)\times (n+m)}$ for some $m \ge 0$ such that 

\begin{enumerate}
    \item The $\size(\mU) \le \size(\mL)-2|\mL_{i_0, j_0}|+s$. 
    %\yufan{Should we define $|x|$ for $x \in \mathbb{Z}_p$ in section 2? We use it here as well.} 
    \label{itm:replaceitem1}
    \item For any non-diagonal entry $\mL_{i, j}$ where $(i, j)\in [n]\times[n]$ except  $(i_0, j_0)$ and $(j_0, i_0)$, $\mU_{i, j}=\mL_{i, j}$.
    \label{itm:replaceitem2}
    \item For any linear system $\mL \vx = \vb$, $\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\mU \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}$.
    \label{itm:replaceitem3}
\end{enumerate}
\end{lemma}
\begin{proof}
    Without loss of generality, we may assume $i_0=1$ and $j_0=2$. Suppose $\mR$ is a $k$ by $k$ matrix. Define 
    \[
    \mU=\left[\begin{array}{cccc}
    \mL_{1, 1}+\mL_{1, 2} +\mR_{1, 1} & \mR_{1, 2} & \mL_{1, 3:n} & \mR_{1, 3:k} \\
    \mR_{2, 1} & \mL_{2, 2}+\mL_{1, 2}+\mR_{2, 2} & \mL_{2, 3:n} & \mR_{2, 3:k} \\
    \mL_{3:n, 1} & \mL_{3:n, 2} & \mL_{3:n, 3:n} & \vzero\\
    \mR_{3:k, 1} & \mR_{3:k, 2}  & \vzero & \mR_{3:k, 3:k}\\
    \end{array}\right].
    \] 
    Item \ref{itm:replaceitem1} and Item \ref{itm:replaceitem2} follows from the definition directly.
    Let $m=k-2, S = \{n+1, \ldots, n+m\}$. We have 
    \begin{align*}
        \quad \sc(\mU, [n])
        &=\mU_{[n], [n]} - \mU_{1:2, S} \mU_{S, S}^{-1} \mU_{S, 1:2}\\
        &=\left(\mU_{[n], [n]}-\mR_{1:2, 1:2}\right) 
        + \mR_{1:2, 1:2} -\mU_{1:2, S} \mU_{S, S}^{-1} \mU_{S, 1:2}\\
        &=\left(\mU_{[n], [n]}-\mR_{1:2, 1:2}\right) +\mR_{1:2, 1:2} 
        -\mR_{1:2, 3:k} \mR_{3:k, 3:k}^{-1} \mR_{3:k, 1:2}\\
        &= \left(\mU_{[n], [n]}-\mR_{1:2, 1:2}\right)+\sc(\mR, \{1, 2\})\\
        &= \left(\mL_{[n], [n]}+\vchi_{1, 2}^\top \mL_{1, 2} \vchi_{1, 2}\right)+\sc(\mR, \{1, 2\})\\
        %&= \mL_{[n], [n]}\\
        &=\mL.
    \end{align*}
    %\begin{align*}
    %    &\sc(\mU, [n])\\
    %    =&\mU_{[n], [n]} - \mU_{1:2, n+1:n+m} \mU_{n+1:n+m, n+1:n+m]]}^{-1} \mU_{n+1:n+m, 1:2}\\
    %    =&\mR_{[\{1, 2\}, \{1, 2\}]} + \left(\mU_{[[n], [n]]}-\mR_{[\{1, 2\}, \{1, 2\}]}\right) \\
    %    &-\mU_{[\{1, 2\}, [n+1, n+m]]} \mU_{[[n+1, n+m], [n+1, n+m]]}^{-1} \mU_{[[n+1, n+m], \{1, 2\}]}\\
    %    =&\mR_{[\{1, 2\}, \{1, 2\}]} + \left(\mU_{[[n], [n]]}-\mR_{[\{1, 2\}, \{1, 2\}]}\right) \\
    %    &-\mR_{[\{1, 2\}, [3, k]]} \mR_{[[3, k], [3, k]]}^{-1} \mR_{[[3, k], \{1, 2\}]}\\
    %    =& \left(\mU_{[[n], [n]]}-\mR_{[\{1, 2\}, \{1, 2\}]}\right)+\sc(\mR, \{1, 2\})\\
    %    =& \left(\mL_{[[n], [n]]}+\vchi_{1, 2}^\top \mL_{1, 2} \vchi_{1, 2}\right)+\sc(\mR, \{1, 2\})\\
    %    =& \mL_{[[n], [n]]}\\
    %    =&\mL.
    %\end{align*}
    Since $\sc(\mU, [n])=\mL$, Item \ref{itm:replaceitem3} follows from Lemma \ref{lem:sc_preserve_sol_1} and Lemma \ref{lem:sc_preserve_sol_2}.
\end{proof}


%\yufan{we need to be careful here. We only use para and seri to construct useful resistor networks, i.e. if $(a+b)^{-1}$ doesn't exist, we don't construct that network since it's useless for our reduction. This assumption makes sure that SC always exists}
\subsection{Connecting Circuits in Parallel or in Series}
To reduce a Laplacian system to a unit-weight Laplacian system, Lemma~\ref{lem:replace_edge} shows that it is enough to construct a circuit consisting of unit-weight edges with certain resistance. Our construction depends on the following physical rule of connecting circuits in parallel or in series. It is forklore for $\mathbb{R}$. We reprove it for $\mathbb{Z}_p$ for completeness.
\begin{lemma}
\label{lem:pa_and_se}
Let $\mL \in \mathbb{Z}^{n\times n}_p$ and $\mU \in \mathbb{Z}^{m\times m}_p$ be two circuits with resistance $a$ and $b$, respectively. Then 
\begin{enumerate}
    \item There exists a circuit $\parallel(\mL, \mU)\in \mathbb{Z}^{(n+m-1)\times (n+m-1)}_p$ such that 
    \begin{enumerate}
        \item The resistance of $\parallel(\mL, \mU)$ is $\frac{ab}{a+b}$.
        \item $\size(\parallel(\mL, \mU))\le \size(\mL)+\size(\mU)$.
    \end{enumerate}\label{itm:parallel}
    \item There exists a circuit $\series(\mL, \mU)\in \mathbb{Z}^{(n+m-2)\times (n+m-2)}_p$ such that 
    \begin{enumerate}
        \item The resistance of $\series(\mL, \mU)$ is $a+b$.
        \item $\size(\series(\mL, \mU))\le \size(\mL)+\size(\mU)$.
    \end{enumerate}\label{itm:series}
\end{enumerate}
\end{lemma}
%\input{appendix_schur.tex}


\begin{proof}

Proof for Item \ref{itm:series}: Define 
\begin{align*}
\series(\mL, \mU)\defeq \left[
\begin{array}{ccccc}
\mL_{1, 1} & 0 &  \mL_{1, 2}&\mL_{1, 3:n}& \vzero \\
0&\mU_{1, 1}&\mU_{1, 2}&\vzero & \mU_{1, 3:m}\\
\mL_{2, 1}&\mU_{2, 1} & \mL_{2, 2}+\mU_{2, 2} & \mL_{2, 3:n} &\mU_{2, 3:m} \\
\mL_{3:n, 1}& \vzero &  \mL_{3:n, 2} & \mL_{3:n, 3:n} & \vzero\\
\vzero& \mU_{3:m, 1} & \mU_{3:m, 2} & \vzero & \mU_{3:m, 3:m} \\
\end{array}\right].
\end{align*}
Let $T=\{1, 2, 3\}, F=\{4, \ldots, n+m-2\}$. $\size(\series(\mL, \mU))\le \size(\mL)+\size(\mU)$ is satisfied
because $\size(\mA)+\size(\mB)\ge \size(\mA+\mB)$ for any matrices $\mA, \mB$ over $\mathbb{Z}_p$. By definition, we have  
\begin{align*}
    & \quad \sc(\series(\mL, \mU), \{1, 2, 3\})\\
    &= \series(\mL, \mU)_{T, T}-\series(\mL, \mU)_{T, F}
    \series(\mL, \mU)_{F, F}^{-1}
    \series(\mL, \mU)_{F, T}\\
    &=\left[
    \begin{array}{ccc}
    \mL_{1, 1} & 0  & \mL_{1, 2}\\ 
    0 & \mU_{1, 1} & \mU_{1, 2} \\
    \mL_{2, 1} & \mU_{2, 1} & \mL_{2, 2} + \mU_{2, 2}
    \end{array}
    \right]
    -\left[
    \begin{array}{cc}
    \mL_{1, 3:n}& \vzero \\
    \vzero & \mU_{1, 3:m} \\
    \mL_{2, 3:n} &\mU_{2, 3:m}
    \end{array}
    \right]
    \left[
    \begin{array}{cc}
    \mL_{3:n, 3:n} & \vzero\\
    \vzero & \mU_{3:m, 3:m}
    \end{array}
    \right]^{-1}
    \left[
    \begin{array}{ccc}
    \mL_{3:n, 1}& 0 & \mL_{3:n, 2}\\
    0& \mU_{3:m, 1}&\mU_{3:m, 2}
    \end{array}\right]\\
    &=\left[
    \begin{array}{ccc}
    \mL_{1, 1} & 0  & \mL_{1, 2}\\
    0 & \mU_{1, 1} & \mU_{1, 2} \\
    \mL_{2, 1} & \mU_{2, 1} & \mL_{2, 2} + \mU_{2, 2}
    \end{array}
    \right]
    -\left[
    \begin{array}{ccc}
    \mL_{1, 3:n} \mL_{3:n, 3:n}^{-1} \mL_{3:n, 1} & \vzero & \mL_{1, 3:n}\mL_{3:n, 3: n}^{-1} \mL_{3:n, 2}\\
    \vzero & \mU_{1, 3:m}\mU_{3:m, 3:m}^{-1} \mU_{3:m, 1} & \mU_{1, 3:m}\mU_{3:m, 3:m}^{-1} \mU_{3:m, 2}\\
    \mL_{2, 3:n}\mL_{3:n, 3:n}^{-1} \mL_{3:n, 1} & \mU_{2, 3:m}\mU_{3:m, 3:m}^{-1} \mU_{3:m, 1} & \left(\makecell{\mL_{2, 3:n}\mL_{3:n, 3:n}^{-1} \mL_{3:n, 2}\\+\\\mU_{2, 3:m}\mU_{3: m, 3:m}^{-1} \mU_{3:m, 2}}\right)
    \end{array}\right]\\
    &=\left[\begin{array}{ccc}\sc(\mL, \{1, 2\})_{1, 1} & 0 & \sc(\mL, \{1, 2\})_{1, 2}\\ 0 &\sc(\mU, \{1, 2\})_{1, 1} & \sc(\mU, \{1, 2\})_{1, 2}\\ \sc(\mL, \{1, 2\})_{2, 1}  & \sc(\mU, \{1, 2\})_{2, 1} & \sc(\mL, \{1, 2\})_{2, 2}+\sc(\mU, \{1, 2\})_{2, 2}\end{array}\right]\\
    &=\left[\begin{array}{ccc}a^{-1} & 0 & -a^{-1}\\ 0 &b^{-1} & -b^{-1}\\ -a^{-1}  & -b^{-1} & a^{-1}+b^{-1}\end{array}\right].
\end{align*}
%\begin{align*}
%    &\sc(\series(\mL, \mU), \{1, 2, 3\})\\
%    =& (\series(\mL, \mU))_{[T, T]}-\series(\mL, \mU)_{[T, F]}
%    \series(\mL, \mU)_{[F, F]}^{-1}
%    \series(\mL, \mU)_{[F, T]}\\
%    =&\left[\begin{array}{ccc}\mL_{1, 1} & 0  & \mL_{1, 2}\\ 0 & \mU_{1, 1} & \mU_{1, 2} \\ \mL_{2, 1} & \mU_{2, 1} & \mL_{2, 2} + \mU_{2, 2}\end{array}\right]\\
%    &-\left[\begin{array}{cc}\mL_{[1, [3,n]]}& \vzero \\\vzero & \mU_{[1, [3, m]]} \\  \mL_{[2, [3,n]]} &\mU_{[2, [3, m]]} \end{array}\right]
%    \left[\begin{array}{cc}\mL_{[[3, n], [3, n]]} & \vzero\\
%\vzero & \mU_{[[3, m], [3, m]]} \end{array}\right]^{-1}
%    \left[\begin{array}{ccc}\mL_{[[3,n], 1]}& 0& \mL_{[[3,n], 2]}\\ 0& \mU_{[[3, m], 1]}&\mU_{[[3, m], 2]}\end{array}\right]\\
%    =&\left[\begin{array}{ccc}\mL_{1, 1} & 0  & \mL_{1, 2}\\ 0 & \mU_{1, 1} & \mU_{1, 2} \\ \mL_{2, 1} & \mU_{2, 1} & \mL_{2, 2} + \mU_{2, 2}\end{array}\right]\\
%    &-\left[\begin{array}{ccc}\mL_{[1, [3,n]]}\mL_{[[3, n], [3, n]]}^{-1} \mL_{[[3,n], 1]} & \vzero & \mL_{[1, [3,n]]}\mL_{[[3, n], [3, n]]}^{-1} \mL_{[[3,n], 2]}\\
%    \vzero & \mU_{[1, [3,m]]}\mU_{[[3, m], [3, m]]}^{-1} \mU_{[[3,m], 1]} & \mU_{[1, [3,m]]}\mU_{[[3, m], [3, m]]}^{-1} \mU_{[[3,m], 2]}\\
%    \mL_{[2, [3,n]]}\mL_{[[3, n], [3, n]]}^{-1} \mL_{[[3,n], 1]} & \mU_{[2, [3,m]]}\mU_{[[3, m], [3, m]]}^{-1} \mU_{[[3,m], 1]} & \left(\makecell{\mL_{[2, [3,n]]}\mL_{[[3, n], [3, n]]}^{-1} \mL_{[[3,n], 2]}\\+\mU_{[2, [3,m]]}\mU_{[[3, m], [3, m]]}^{-1} \mU_{[[3,m], 2]}}\right)
%    \end{array}\right]\\
%    =&\left[\begin{array}{ccc}\sc(\mL, \{1, 2\})_{1, 1} & 0 & \sc(\mL, \{1, 2\})_{1, 2}\\ 0 &\sc(\mU, \{1, 2\})_{1, 1} & \sc(\mU, \{1, 2\})_{1, 2}\\ \sc(\mL, \{1, 2\})_{2, 1}  & \sc(\mU, \{1, 2\})_{2, 1} & \sc(\mL, \{1, 2\})_{2, 2}+\sc(\mU, \{1, 2\})_{2, 2}\end{array}\right]\\
%    =&\left[\begin{array}{ccc}a^{-1} & 0 & -a^{-1}\\ 0 &b^{-1} & -b^{-1}\\ -a^{-1}  & -b^{-1} & a^{-1}+b^{-1}\end{array}\right].
%\end{align*}
By Lemma \ref{lem:commutative}, 
\begin{align*}
    & \quad \sc(\series(\mL, \mU), \{1, 2\})\\
    &=\sc(\sc(\series(\mL, \mU), \{1, 2, 3\}), \{1, 2\})\\
    &=\sc\left(\left[
    \begin{array}{ccc}
    a^{-1} & 0 & -a^{-1}\\
    0 &b^{-1} & -b^{-1}\\
    -a^{-1}  & -b^{-1} & a^{-1}+b^{-1}\end{array}\right]
    , \{1, 2\}\right)\\
    &=\left[\begin{array}{cc}\frac{1}{a+b} & -\frac{1}{a+b}\\ -\frac{1}{a+b} &\frac{1}{a+b}\end{array}\right].
\end{align*}
Proof for Item \ref{itm:parallel}:
Define 
\begin{align*}
\parallel(\mL, \mU)\defeq \left[
\begin{array}{cccc}
\multicolumn{2}{c}{\multirow{2}{*}{$\mL_{1:2, 1:2}+\mU_{1:2, 1:2}$}}& \mL_{1, 3:n} & \mU_{1, 3:m} \\
\multicolumn{2}{c}{}& \mL_{2, 3:n}& \mU_{2, 3:m} \\
\mL_{3:n, 1} & \mL_{3:n, 2}  & \mL_{3:n, 3:n} & \vzero\\
\mU_{3:m, 1} & \mU_{3:m, 2}  & \vzero & \mU_{3:m, 3:m}
\end{array}\right].
\end{align*}
%\begin{align*}
%\parallel(\mL, \mU)\defeq \left[
%\begin{array}{cccc}
%\multicolumn{2}{c}{\multirow{2}{*}{$\mL_{[\{1, 2\}, \{1, 2\}]}+\mU_{[\{1, 2\}, \{1, 2\}]}$}}& \mL_{[1, [3, n]]} & \mU_{[1, [3, m]]} \\
%\multicolumn{2}{c}{}& \mL_{[2, [3, n]]}& \mU_{[2, [3, m]]} \\
%\mL_{[[3, n], 1]} & \mL_{[[3, n], 2]}  & \mL_{[[3,n], [3,n]]}& \vzero\\
%\mU_{[[3, m], 1]} & \mU_{[[3, m], 2]}  & \vzero & \mU_{[[3,m], [3,m]]}
%\end{array}\right].
%\end{align*}
 $\size(\parallel(\mL, \mU))\le \size(\mL)+\size(\mU)$ is satisfied for the same reason as in Item \ref{itm:series}. Let $T=\{1, 2\}, F=\{3, \ldots, n+m-2\}$. By definition, we have 
\begin{align*}
    & \quad \sc(\parallel(\mL, \mU), \{1, 2\})\\
    &= (\mL+\mU)_{T, T}-\parallel(\mL, \mU)_{T, F}
    \parallel(\mL, \mU)_{F, F}^{-1}
    \parallel(\mL, \mU)_{F, T}\\
    &=(\mL+\mU)_{T, T}-\left[\begin{array}{cc}\mL_{1, 3:n} & \mU_{1, 3:m}\\ \mL_{2, 3: n}&\mU_{2, 3:m}\end{array}\right]
    \left[\begin{array}{cc}\mL_{3:n, 3:n} & \vzero \\ \vzero & \mU_{3:m, 3: m}\end{array}\right]^{-1}
    \left[\begin{array}{cc}\mL_{3:n, 1} & \mL_{3:n, 2}\\\mU_{3:m, 1} & \mU_{3:m, 2}\end{array}\right]\\
    &=(\mL+\mU)_{T, T}-\left(\mL_{1:2, 3:n} \mL_{3:n, 3:n}^{-1} \mL_{3:n, 1:2} + \mU_{1:2, 3:m} \mU_{3:m, 3:m}^{-1} \mU_{3:m, 1:2}\right)\\
    &=\sc(\mL, \{1, 2\})+\sc(\mU, \{1, 2\})\\
    &=\vchi_{1, 2}^\top (a^{-1}+b^{-1}) \vchi_{1, 2} \qedhere
\end{align*}
%\begin{align*}
%    &\sc(\parallel(\mL, \mU), \{1, 2\})\\
%    =& (\mL+\mU)_{[T, T]}-\parallel(\mL, \mU)_{[T, F]}
%    \parallel(\mL, \mU)_{[F, F]}^{-1}
%    \parallel(\mL, \mU)_{[F, T]}\\
%    =&(\mL+\mU)_{[T, T]}-\left[\begin{array}{cc}\mL_{[1, [3, n]]} & \mU_{[1, [3, m]]}\\ \mL_{[2, [3, n]]}&\mU_{[2, [3, m]]}\end{array}\right]
%    \left[\begin{array}{cc}\mL_{[[3, n], [3, n]]} & \vzero \\ \vzero & \mU_{[[3, m], [3, m]]}\end{array}\right]^{-1}
%    \left[\begin{array}{cc}\mL_{[[3, n], 1]} & \mL_{[[3, n], 2]}\\\mU_{[[3, m], 1]} & \mU_{[[3, m], 2]}\end{array}\right]\\
%    =&(\mL+\mU)_{[T, T]}-\left(\mL_{[\{1, 2\}, [3, n]]} \mL_{[[3, n], [3, n]]}^{-1} \mL_{[[3, n], \{1,2\}]} + \mU_{[\{1, 2\}, [3, m]]} \mU_{[[3, m], [3, m]]}^{-1} \mU_{[[3, m], \{1,2\}]}\right)\\
%    =&\sc(\mL, \{1, 2\})+\sc(\mU, \{1, 2\})\\
%    =&\vchi_{1, 2}^\top (a^{-1}+b^{-1}) \vchi_{1, 2} \qedhere
%\end{align*}
\end{proof}


==> stoc22/sec4_2.tex <==

\begin{theorem}
Given any Laplacian system $\mL \in \mathbb{Z}_p^{n\times n}$, we can compute a Laplacian system $\mU \in \mathbb{Z}_p^{k\times k}$ for some $k \le O(pn)$ such that 
\begin{enumerate}
    \item $size(\mU)\le \nnz(\mL)O(p)$.
    \item Any non-diagonal entry $\mU_{i, j}$ is either $0$ or $-1$.
    \item For any linear system $\mL \vx = \vb$, $\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\mU \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}$.
\end{enumerate}
\end{theorem}

\begin{lemma}
\label{lem:resistance_construction_p}
Let $r$ be an integer in $[1, p-1]$. There exists a circuit with size $O(p)$ and resistance $r$.

\end{lemma}
\begin{proof}
We define $\mU_i$ recursively: 
\begin{itemize}
    \item $\mU_i=\series(\mU_{i-1}, \mU_1)$ for $i>1$.
    \item $\mU_1$ is the unit circuit $\vchi_{1, 2}^\top \vchi_{1, 2}$.
\end{itemize}
By applying Lemma \ref{lem:pa_and_se} inductively, $\mU_r$ is the desired circuit.
\end{proof}


%Since when $p = 2$, any Laplacian matrix is naturally a unit weight Laplacian matrix, we only consider the case $p \ge 3$. Let $k = 2(p - 1 - \mL_{i_0, j_0})$, consider the matrix 
%\begin{align*}
%    \mU = 
%    \left[
%    \begin{array}{cc}
%       \mU_{T,T}  & \mU_{T, S} \\
%       \mU_{S,T}  & \mU_{S, S} \\ 
%    \end{array}
%    \right]
%    =
%    \left[
%    \begin{array}{cc}
%       \mL + (\ve_{i_0} + \ve_{j_0}) \vone_k^T 2^{p-2} \eye_k \vone_k (\ve_{i_0} + \ve_{j_0})^T  &  -(\ve_{i_0} + \ve_{j_0}) \vone_k^T\\
%       -\vone_k (\ve_{i_0} + \ve_{j_0})^T  & 2 \eye_k \\ 
%    \end{array}
%    \right]
%\end{align*}
%where $T = [n], S = [n + k] \setminus T$.
%
%\begin{lemma}
%The inverse of $\mU_{S,S} = 2 \eye_k$ exists and\ $\mU_{S,S}^{-1} \equiv 2^{p-2} \eye_k \mod p$.
%\end{lemma}
%\begin{proof}
%    By Fermat's little theorem, $a^{p-1} \equiv 1 \mod p$ for any $a, p$ such that $p$ is a prime and $a$ is coprime with $p$. As we assume $p \ge 3$, 
%    \begin{align*}
%        2^{p-2} \eye_k \mU_{S,S} \equiv 2^{p-1} \eye_k \equiv \eye_k \mod p
%    \end{align*}
%    implies $\mU_{S,S}^{-1} \equiv 2^{p-2} \eye_k \mod p$.
%\end{proof}
%
%\begin{lemma}
%    $\mU$ is a Laplacian matrix over $\mathbb{Z}_p$.
%\end{lemma}
%
%\begin{proof}
%It's easy to verify $\mU$ is symmetric and we have
%\begin{align*}
%    \mU \vone_{n+k} &= 
%    \left[
%    \begin{array}{cc}
%       \mL + (\ve_{i_0} + \ve_{j_0}) \vone_k^T 2^{p-2} \eye_k \vone_k (\ve_{i_0} + \ve_{j_0})^T  &  -(\ve_{i_0} + \ve_{j_0}) \vone_k^T\\
%       -\vone_k (\ve_{i_0} + \ve_{j_0})^T  & 2 \eye_k \\ 
%    \end{array}
%    \right]
%    \vone_{n+k} \\
%    &= 
%    \left[
%    \begin{array}{cc}
%       \mL \vone_n + (\ve_{i_0} + \ve_{j_0}) \vone_k^T 2^{p-2} \eye_k \vone_k (\ve_{i_0} + \ve_{j_0})^T \vone_n  -  (\ve_{i_0} + \ve_{j_0}) \vone_k^T \vone_k\\
%       -\vone_k (\ve_{i_0} + \ve_{j_0})^T \vone_n  + 2 \eye_k \vone_k \\ 
%    \end{array}
%    \right] \\
%    &=
%    \left[
%    \begin{array}{cc}
%       (\ve_{i_0} + \ve_{j_0}) (2^{p-2} k)(\ve_{i_0} + \ve_{j_0})^T \vone_n  -  (\ve_{i_0} + \ve_{j_0}) k\\
%       -\vone_k (\ve_{i_0} + \ve_{j_0})^T \vone_n  + 2 \eye_k \vone_k \\ 
%    \end{array}
%    \right] \\
%    &=
%    \left[
%    \begin{array}{cc}
%       (\ve_{i_0} + \ve_{j_0}) (2^{p-1} k) -  (\ve_{i_0} + \ve_{j_0}) k\\
%       -2\vone_k + 2 \vone_k \\ 
%    \end{array}
%    \right] \\ 
%    &= \vzero \\
%\end{align*}
%which implies $\mU$ is a Laplacian matrix.
%\end{proof}
%
%\begin{lemma}
%    $\mU_{i, j} = \mL_{i,j}$ for all $(i, j) \in [n] \times [n]$ such that $i \neq j$ and $(i, j) \not\in \{(i_0, j_0), (j_0, i_0)\}$.
%\end{lemma}
%
%\begin{lemma}
%    $\mU_{i, j} \in \{0, -1\}$ for all $(i, j) \in \{(i_0, j_0), (j_0, i_0)\} \bigcup ([n + k] \times [n + k]) \setminus ([n] \times [n])$. 
%\end{lemma}
%
%\begin{lemma}
%    As $\mU_{S,S}^{-1}$ exists, $\sc(\mU, T) = \mL$.
%\end{lemma}
%
%\begin{corollary}
%    For any linear system $\mL \vx = \vb$, $\left\{\vx\mid \mL \vx = \vb\right\}=\left\{\vy_{[n]}\mid\mU \vy = \left[\begin{array}{c}\vb \\ \vzero \end{array}\right]\right\}$.
%\end{corollary}
